$U(1)$ local strings in hybrid metric-Palatini gravity

In this work we made use of a general static cillindrically symmetric metric to find $U(1)$ local cosmic string solutions in the context of the hybrid metric-Palatini theory of gravity in it's scalar-tensor representation. After finding the dynamical equations for this particular case, we imposed boost invariance along $t$ and $z$ directions, which simplified the equations of motions, leaving only one single metric tensor component, $W^2(r)$. For an arbitrary potential $V(\phi)$, the solutions obtained can be put in a closed parametric form, with $\phi$ taken as a parameter. Several particular cases of the potential were studied, some yielding simple mathematical forms, others with only numerical solutions. With this approach, we obtain a large number of new stable stringlike solutions in hybrid metric-Palatini gravity, in which the parameters, like the scalar field, metric tensor components, and string tension, depend fundamentally on the boundary values of the scalar field, and its derivative, on the $r(0)$ circular axis.

==> main-references.tex <==
%\cite{Zee:2003mt}
\bibitem{Zee:2003mt}
A.~Zee,
%``Quantum field theory in a nutshell,''
%180 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Utiyama:1962sn}
\bibitem{Utiyama:1962sn}
R.~Utiyama and B.~S.~DeWitt,
%``Renormalization of a classical gravitational field interacting with quantized matter fields,''
J. Math. Phys. \textbf{3} (1962), 608-618
doi:10.1063/1.1724264
%414 citations counted in INSPIRE as of 28 Oct 2021

%\cite{Lovelock:1971yv}
\bibitem{Lovelock:1971yv}
D.~Lovelock,
%``The Einstein tensor and its generalizations,''
J. Math. Phys. \textbf{12} (1971), 498-501
doi:10.1063/1.1665613
%2000 citations counted in INSPIRE as of 28 Oct 2021

%\cite{Harko:2011nh}
\bibitem{Harko:2011nh}
T.~Harko, T.~S.~Koivisto, F.~S.~N.~Lobo and G.~J.~Olmo,
%``Metric-Palatini gravity unifying local constraints and late-time cosmic acceleration,''
Phys. Rev. D \textbf{85} (2012), 084016
doi:10.1103/PhysRevD.85.084016
[arXiv:1110.1049 [gr-qc]].
%138 citations counted in INSPIRE as of 18 Oct 2021

%\cite{Harko:2020ibn}
\bibitem{Harko:2020ibn}
T.~Harko and F.~S.~N.~Lobo,
%``Beyond Einstein\textquoteright{}s General Relativity: Hybrid metric-Palatini gravity and curvature-matter couplings,''
Int. J. Mod. Phys. D \textbf{29} (2020) no.13, 2030008
doi:10.1142/S0218271820300086
[arXiv:2007.15345 [gr-qc]].
%20 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Vilenkin:2000jqa}
\bibitem{Vilenkin:2000jqa}
A.~Vilenkin and E.~P.~S.~Shellard,
%``Cosmic Strings and Other Topological Defects,''
%47 citations counted in INSPIRE as of 17 Oct 2021

%\cite{Olmo:2011uz}
\bibitem{Olmo:2011uz}
G.~J.~Olmo,
%``Palatini Approach to Modified Gravity: f(R) Theories and Beyond,''
Int. J. Mod. Phys. D \textbf{20} (2011), 413-462
doi:10.1142/S0218271811018925
[arXiv:1101.3864 [gr-qc]].
%462 citations counted in INSPIRE as of 29 Oct 2021

%\cite{Vilenkin:1981zs}
\bibitem{Vilenkin:1981zs}
A.~Vilenkin,
%``Gravitational Field of Vacuum Domain Walls and Strings,''
Phys. Rev. D \textbf{23} (1981), 852-857
doi:10.1103/PhysRevD.23.852
%997 citations counted in INSPIRE as of 25 Oct 2021

%\cite{ATLAS:2015yey}
\bibitem{ATLAS:2015yey}
G.~Aad \textit{et al.} [ATLAS and CMS],
%``Combined Measurement of the Higgs Boson Mass in $pp$ Collisions at $\sqrt{s}=7$ and 8 TeV with the ATLAS and CMS Experiments,''
Phys. Rev. Lett. \textbf{114} (2015), 191803
doi:10.1103/PhysRevLett.114.191803
[arXiv:1503.07589 [hep-ex]].
%1919 citations counted in INSPIRE as of 29 Oct 2021
